LaRS: A Diverse Panoptic Maritime Obstacle Detection Dataset and Benchmark

The progress in maritime obstacle detection is hindered by the lack of a diverse dataset that adequately captures the complexity of general maritime environments. We present the first maritime panoptic obstacle detection benchmark LaRS, featuring scenes from Lakes, Rivers and Seas. Our major contribution is the new dataset, which boasts the largest diversity in recording locations, scene types, obstacle classes, and acquisition conditions among the related datasets. LaRS is composed of over 4000 per-pixel labeled key frames with nine preceding frames to allow utilization of the temporal texture, amounting to over 40k frames. Each key frame is annotated with 8 thing, 3 stuff classes and 19 global scene attributes. We report the results of 27 semantic and panoptic segmentation methods, along with several performance insights and future research directions. To enable objective evaluation, we have implemented an online evaluation server. The LaRS dataset, evaluation toolkit and benchmark are publicly available at: https://lojzezust.github.io/lars-dataset

==> cutout.tex <==
INTRO:
------------------------------------------------------------------------------------------------------------
% What is maritime obstacle detection and why it is needed
% Current state of the art is semantic segmentation
% Lack of per-pixel labeled datasets, datasets lack variety (mostly captured in a single location)
% Why is panoptic segmentation needed? Semantic segmentation does not detect individual dynamic obstacles
% We present LaRS, a new panoptic dataset, large variety of aquatic scenes (lakes, rivers and seas), different obstacle types annotated, focus on hazardous examples
% We propose an evaluation protocol for evaluating panoptic and semantic segmentation mehtods
% We evaluate a large number of semantic and panoptic segmentation baselines (state-of-the-art)



%Maritime obstacle detection is a crucial task for ensuring the safe navigation of vessels in aquatic environments and enabling the autonomy of both small and large unmanned surface vehicles (USVs). It plays a vital role in a wide range of potential use cases, including automated inspection, environmental monitoring, waste cleanup, cargo shipping, and ferry transport, and is essential for avoiding collisions, delays, and costly accidents. 

%In this study, we focus on camera-based obstacle detection, which uses visual data from cameras to detect obstacles in aquatic environments. This approach is particularly appealing due to the widespread availability and low cost of cameras, as well as their demonstrated potential in various computer vision tasks in recent years (TODO). With the proliferation of affordable cameras on smartphones, drones, and other devices, it is now also possible to collect large amounts of visual data at low cost, making it an attractive choice for researchers and practitioners working in the field. The camera-based approach also has several advantages over other modalities, such as RADAR or LIDAR, which may be limited by range, resolution, or interference from environmental factors.

Automation is increasingly transforming the maritime industry. With over ??\% of goods being moved over water, substantial efforts are being invested in autonomous surface vessels~\cite{?,?}, which cater diverse applications, ranging from automated inspection, environmental monitoring, waste cleanup, cargo shipping, and human transport. Among several challenges in maritime navigation, obstacle detection is one of the most crucial for timely collision avoidance and harm prevention.

%Maritime obstacle detection is a crucial task for ensuring safe navigation of autonomous surface vehicles~\cite{Bovcon2020MODS}.  It plays crucial role in both small and large unmanned surface vehicles (USVs)~\cite{Bovcon2020MODS}. It plays a vital role in a range of applications, including automated inspection, environmental monitoring, waste cleanup, cargo shipping, and ferry transport, and is essential for avoiding collisions, delays, and costly accidents.

%Significant advancements have been made recently in camera-based obstacle detection~\cite{Bovcon2018Stereo,Cane2019Evaluating,Prasad2019Object}, which, compared to modalities like RADAR and LIDAR, bear several advantages such as being high-resolution, light-weight, cost-effective and information-rich sensors. 
  
Similarly to the automotive domain~\cite{?}, cameras, as cost-effective and information-rich sensors, have been extensively explored for this problem~\cite{Kristan2016Fast,Bovcon2018Stereo,Cane2019Evaluating,Prasad2019Object}, posing the problem either as a bounding-box detection of objects of known obstacle classes (\eg ships, swimmers) or a semantic-segmentation-based parsing of the scene into navigable (\ie water) and non-navigable (\ie obstacles) regions.
% Maritime obstacle detection is a crucial task for the safe navigation of USVs. Over the past few years, marine perception has followed the trend in autonomous ground vehicles (AGV) by adopting segmentation-based deep learning methods for obstacle detection, treating the problem as anomaly segmentation and assigning all obstacles (static and dynamic) to a single obstacle class. However, the dynamic nature of the water surface and reflections in the maritime domain make it difficult to directly apply AGV-based semantic segmentation models~\cite{Chen2017Rethinking,Yu2021BiSeNet} to this domain~\cite{Bovcon2019Mastr,Cane2019Evaluating}, resulting in high recall rates of obstacles but low precision, struggling to handle the changing appearance of the water surface.

%While the initial methods were statistical~\cite{Kristan2016Fast,Cane?}, the modern methods rely on deep learning 

%To address static obstacles such as shores and dynamic obstacles like boats, the state-of-the-art~\cite{Bovcon2021WaSR,Yao2021Shoreline,Qiao2022Automated,Zust2022Temporal} casts obstacle detection as semantic segmentation of the image into water, obstacles and sky pixels.

%The current state-of-the-art~\cite{?,?,?} is based on sematic segmentation, where the image is split into water, sky and obstacle pixels. 



\begin{figure}
  \centering
  \includegraphics[width=\linewidth]{figures/lars_ex.pdf}
  \caption{LaRS features a large number of diverse and challenging USV-centric scenes with per-pixel panoptic obstacle segmentation annotations (bottom right).}
    \label{fig:motivation}
\end{figure}


%The current state-of-the-art approaches for maritime obstacle detection pose the problem as semantic segmentation, where the goal is to assign a class label (\ie water, sky or obstacle) to each pixel in an image. While this approach has been successful in many applications (TODO), it has several limitations when it comes to detecting dynamic obstacles in aquatic environments. In particular, semantic segmentation is not capable of identifying individual instances of obstacles, which is highly desirable from the USV navigation perspective to enable the tracking and planing for paths of obstacles, and is prone to confusion on reflections and situations when the appearance of an obstacle is similar to that of the surrounding environment.

%The development of obstacle segmentation methods is further hindered by the lack of per-pixel annotated datasets. While many datasets provide bounding box annotations for individual objects in the scene, relatively few contain per-pixel labels suitable for training and evaluation of segmentation methods and only one provides panoptic labels. Furthermore, as most maritime datasets have a very restricted regional coverage, with images captured in a single harbor or canal, they lack the visual variety required for training and evaluation of robust obstacle detection, resilient to environment-specific situations such as reflections on still lakes and narrow waterways of canals.

Several evaluation datasets~\cite{Prasad2017Video,Bovcon2018Stereo,Bovcon2020MODS} have been proposed to facilitate the development of camera-based obstacle detection methods (see Table~\ref{tab:datasets}). However, these datasets employ object bounding box annotations, which limits the ability to evaluate the performance of segmentation-based methods. The development of segmentation methods is further hampered by the limited scope of existing segmentation datasets~\cite{Bovcon2019Mastr,Cheng2021Are}, which are usually captured within very localized geographical areas, lack the visual variety required for general and robust obstacle detection and are mostly small scale, containing less than 1000 annotated images. Recent work~\cite{?} also shows the benefit of using temporal information from recent image frames for improved robustness in challenging scenarios, which is not provided in most existing datasets.


While background static obstacles (\eg piers, shore) are principally addressed by semantic segmentation, the dynamic obstacles can also be treated as objects. In fact, the recent maritime benchmark~\cite{Bovcon2020MODS} has shown benefits of using object detectors for dynamic obstacles. Panoptic segmentation~\cite{Kirillov2019Panoptic} jointly addresses both tasks and has shown significant promise in camera-based perception methods for autonomous vehicles~\cite{Cheng2020Panoptic,Cheng2021Mask2Former,Zendel2022Unifying}. 
However, development of maritime panoptic segmentation methods is hampered by the lack publicly available training and testing datasets.

We address the aforementioned drawbacks by proposing the first RGB maritime panoptic obstacle detection benchmark. Our first major contribution is the \underline{La}kes \underline{R}ivers and \underline{S}eas (LaRS) dataset. 
Compared to existing datasets, LaRS boasts the largest diversity in locations, obstacles and acquisition conditions. The dataset is composed of over 4k key frames panoptically annotated by 13 stuff and thing labels and 19 global scene-type attributes. Each key-frame is equipped with preceding nine frames to facilitate development of methods exploiting temporal texture.
The training, validation and test splits were carefully constructed to ensure equal attribute distribution, and an online evaluation server has been implemented to mitigate test-set overfitting.
 
Our second contribution is analysis of 17 recent semantic segmentation networks and 8 panoptic networks. We outline several limitations of the methods and opportunities for their improvement. The new dataset and benchmark provides an insight into the currents state of maritime obstacle detection and will act as strong cornerstone for the future development of the field. The dataset, server and the evaluation toolkit will be released publicly.



%Each image is equipped with the past nine frames to allow development of segmentation methods that exploit temporal information, which amounts approximately 40k image frames in total. 

%Each key frame is annotated with panoptic labels. The background (\ie stuff) is segmented into water, sky and static obstacles, while the dynamic obstacles (\ie things) are annotated as 8 different obstacle types. 
%The scenes are additionally annotated with 19 global attributes for detailed analysis. 

%Special care has been taken to ensure equal attribute distribution among the training, validation and the test splits of the dataset. 

% \cmnt{[MK] če bi lahko še številčno podali kake vrednosti koliko večji ali bogatejši je LaRS v primerjavi z drugimi dataseti, bi bilo super.}

%To address these limitations, we introduce LaRS, a new dataset for the task of panoptic segmentation in aquatic environments. LaRS consists of a large collection of more than 4000 aquatic scenes sourced from different sources (\ie public videos, newly captured videos, sequences from existing datasets) and includes visually varied scenes from lakes, rivers, and seas, with manual per-pixel annotations for water, sky, static obstacles and instances of various common dynamic obstacle types. The scenes in LaRS have been carefully selected to feature hazardous situations such as fog, heavy reflections and bad lighting. We also provide a temporal context of 9 preceding frames to facilitate the development of temporal methods for this task. LaRS is currently by far the largest and most varied segmentation dataset for maritime obstacle detection.

%To evaluate the performance of panoptic and semantic segmentation methods on LaRS, we design a new evaluation protocol focused on the important aspects for USV navigation. To demonstrate the utility of LaRS, we train and evaluate a large number of semantic and panoptic segmentation baselines, including state-of-the-art approaches. Our results show that LaRS is a challenging and realistic benchmark for the task of maritime obstacle detection, and it can be used to drive the development of more advanced algorithms in this area.

%To summarize, the main contributions of this paper are: (i) the introduction of LaRS as a new panoptic dataset for the task of maritime obstacle detection, (ii) the proposal of a new evaluation protocol for obstacle segmentation methods, and (iii) the evaluation and analysis of a large number of semantic and panoptic segmentation methods on the dataset. We believe that LaRS will be a valuable resource for researchers and practitioners working in the field of computer vision, and it will help to drive the development of more advanced and practical algorithms for maritime obstacle detection.
------------------------------------------------------------------------------------------------------------
